The Group Loss++: A deeper look into group loss for deep metric learning

Deep metric learning has yielded impressive results in tasks such as clustering and image retrieval by leveraging neural networks to obtain highly discriminative feature embeddings, which can be used to group samples into different classes. Much research has been devoted to the design of smart loss functions or data mining strategies for training such networks. Most methods consider only pairs or triplets of samples within a mini-batch to compute the loss function, which is commonly based on the distance between embeddings. We propose Group Loss, a loss function based on a differentiable label-propagation method that enforces embedding similarity across all samples of a group while promoting, at the same time, low-density regions amongst data points belonging to different groups. Guided by the smoothness assumption that "similar objects should belong to the same group", the proposed loss trains the neural network for a classification task, enforcing a consistent labelling amongst samples within a class. We design a set of inference strategies tailored towards our algorithm, named Group Loss++ that further improve the results of our model. We show state-of-the-art results on clustering and image retrieval on four retrieval datasets, and present competitive results on two person re-identification datasets, providing a unified framework for retrieval and re-identification.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tex_files/ablation_old.tex <==
\begin{table}[htb!]
  \begin{center}
    \label{tab:table1}
        \setlength{\tabcolsep}{1pt}
    \begin{tabular}{l|S S S S S|S S S S S}
     &\multicolumn{5}{c|}{Inshop}& \multicolumn{5}{c|}{SOP}\\
    \hline
      \textbf{inference} & \textbf{R@1} & \textbf{R@10} & \textbf{R@20} & \textbf{R@30} & \textbf{R@40} &\textbf{R@1} & \textbf{R@10} & \textbf{R@100}& \textbf{R@1000}& \textbf{NMI}\\
      \hline
      ap& 86.1 & 96.0 & 97.0 & 97.7 & 98.0&75.4&87.7&94.2&97.9&91.1\\
      mp&87.5& 96.6 & 97.6 & 98.2 & 98.5&75.8&87.9&94.4&97.9&91.1\\
      ap+mp&88.0&96.9&97.8 &98.3&98.5&76.7&88.7&94.9&98.2&91.4\\
      ap+euc&86.8&96.4&97.5&98.0&98.4&76.0&88.2&94.8&98.3&91.3\\
      mp+euc&88.9&97.2&98.2&98.6&98.9&77.7&89.6&95.5&98.4&91.6\\
      ap+mp+euc&89.1&97.2&98.2&98.6&98.9&77.9&89.7&95.6&98.4 &91.7\\
      ap+mp+$\beta$&89.1&97.3&98.2&98.6&98.9&78.0&89.8&95.6&98.4&91.8\\
      ap+mp+$\beta$+lr&89.6&97.5&98.3&98.7&99.0&78.5&90.0&95.8&98.6&92.0\\
      ap+mp+$\beta$+lr+r&90.5&97.5&98.4&98.7&99.0&79.0&90.0&95.8&98.5&92.0\\
      \hline
    \end{tabular}
  \end{center}
        \caption{The influence of different inference configurations on the best performing models achieved using the Group Loss.
        ap=average pooling, mp=max pooling, euc=euclidean normalization,\newline $\beta$-n=$\beta$-normalization, lr=LeakyReLU, r=re-ranking}.
\label{fig:performance_grouploss_ablation}
\end{table}




\begin{table}[htb!]
  \begin{center}
    \label{tab:table1}
        \setlength{\tabcolsep}{1pt}
    \begin{tabular}{l|S S S S S|S S S S S}
     & \multicolumn{5}{c|}{Cars 196} & \multicolumn{5}{c|}{CUB-200-2011}\\
    \hline
      \textbf{inference} & \textbf{R@1} & \textbf{R@2} & \textbf{R@4} & \textbf{R@8} & \textbf{NMI} &\textbf{R@1} & \textbf{R@2} & \textbf{R@4} & \textbf{R@8} & \textbf{NMI}&\\
      \hline
      ap& 83.3 & 89.4 & 93.5 & 95.8 & 69.2 &64.9&75.4&84.0&90.6&68.4\\
      mp&86.3& 91.5 & 94.85 & 96.6 & 69.4 &66.1&77.1&85.4&91.0&68.3\\
      ap+mp&86.4&91.6&94.9 &96.7&70.0 &66.6&77.5&85.3&91.0&69.2\\
      ap+euc&87.0&92.3& 95.6&97.5&72.5&66.8&77.4&85.2&91.3&69.5\\
      mp+euc&88.3&92.8&95.8&97.5&73.0&67.5&78.1&86.2&91.7&70.0\\
      ap+mp+euc&88.4&92.7&95.9&97.5&73.1&67.6&78.3&86.4&91.9&69.7\\
      ap+mp+$\beta$&88.5&92.9&95.9&97.6&73.1&68.0&78.2&86.5&91.5&69.2\\
      ap+mp+$\beta$+lr&88.6&93.1&96.1&97.7&72.5&68.8&78.9&86.6&91.9&70.9\\
      ap+mp+$\beta$+lr+r&89.2&93.2&95.8&97.4&72.5&69.9&78.8&86.0&91.2&70.9\\




      \hline
    \end{tabular}
  \end{center}
        \caption{The influence of different inference configurations on the best performing models achieved using the Group Loss with the proposed training strategy of section 5.3.\newline
        ap=average pooling, mp=max pooling, euc=euclidean normalization,\newline $\beta$-n=$\beta$-normalization, lr=LeakyReLU, r=re-ranking}.
\label{fig:performance_grouploss_ablation}
\end{table}


==> tex_files/comp_sota_cuhk03.tex <==
\begin{table}
\centering
    \resizebox{0.3\textwidth}{!}{%
    \begin{tabular}{@{}l|cc@{}}

\hline
& \multicolumn{2}{c}{CUHK03}  \\
\hline
Method & \textbf{rank-1} & \textbf{rank-5} \\
\hline
PA \cite{DBLP:conf/eccv/SuhWTML18} \textit{ECCV18} & 88.0 & 97.6 \\
CPC \cite{DBLP:conf/cvpr/WangCW018} \textit{CVPR18} & 88.1 & -  \\
MLFN \cite{DBLP:conf/cvpr/ChangHX18} \textit{CVPR18} & 89.2 & - \\
TriNet \cite{DBLP:journals/corr/HermansBL17} & 89.6 & 99.0 \\
GCSL \cite{DBLP:conf/cvpr/Chen0LSW18} \textit{CVPR18} & 90.2 & 98.5  \\
IANet \cite{DBLP:conf/cvpr/HouMCGSC19a} \textit{CVPR19} & 90.1 & 98.2 \\
DKPM \cite{DBLP:conf/cvpr/ShenXLYW18} \textit{CVPR18} & 91.1 & 98.3  \\
MaskBased \cite{DBLP:journals/corr/abs-1804-03864} & 92.3 & - \\
%AlignedReID \parencite{DBLP:journals/corr/abs-1711-08184} & 92.4 & \textbf{\textcolor{blue}{98.9}}  \\
HSP  \cite{DBLP:conf/cvpr/KalayehBGKS18} \textit{CVPR18} & 94.3 & 99.0 \\
DGSRW \cite{DBLP:conf/cvpr/ShenLXYCW18} \textit{CVPR18} & 94.9 & 98.7\\
SGGNN  \cite{DBLP:conf/eccv/ShenLYCW18} \textit{ECCV18} & 95.5 & 99.1 \\
DCDS \cite{DBLP:journals/corr/abs-1904-11397} \textit{ICCV19} & 95.8 & 99.1 \\
\hline
%Ours Resnet50 & 90.0 & 98.4  \\
%Ours (dist 1) & 93.1  & 98.6 \\ 
Group Loss & 88.9 & 97.6 \\
Group Loss + dist & 93.1 & 98.6 \\
Group Loss++ (no RR) & 93.6 & 98.9 \\
%Ours (dist 2) & 93.5 & 98.7 \\

\end{tabular}}

\caption{Comparison to state-of-the-art results on the detected bounding boxes of CUHK03 \cite{DBLP:conf/cvpr/LiZXW14}. \SV{missing bold} }

\label{tab:res_cuhk}

\end{table}


==> tex_files/inference_tricks_reid.tex <==
\begin{table}
\centering
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{@{}l|c|c|c@{}}

\hline
\textbf{} & \multicolumn{1}{c}{Market} & \multicolumn{1}{c}{CUHK03 (NP)} & \multicolumn{1}{c}{CUHK03 (OP)} \\ \hline
\textbf{Method}  &  \textbf{rank-1}  \textbf{mAP} \\ \hline
Ours & 95.0 & 83.4 & 93.5 \\
Ours + Lambda & 95.2 & 83.4 & 93.5 \\
Ours + Lambda + Leak & 95.2 & 83.6 & 93.6\\

\end{tabular}}

\caption{Performance of inference tricks introduced in Section~\ref{sec:inference_tricks} on person re-identification datasets. NP indicates new test protocol, OP old test protocol.}

\label{tab:inference_tricks_reid}

\end{table}

==> tex_files/inshop_gtg_step_ablation.tex <==
\begin{table}[!ht]
\centering
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{@{}l|cccc|cccc@{}}
\hline
\textbf{} & \multicolumn{4}{c}{GroupLoss} & \multicolumn{4}{c}{GroupLoss++} \\ \hline
\textbf{num gtg steps} & \textbf{R@1} & \textbf{R@10} & \textbf{R@20} & \textbf{R@40} & \textbf{R@1} & \textbf{R@10} & \textbf{R@20} & \textbf{R@40} \\ \hline

%0 & 79.2 & 92.7 & 94.7 & 96.2 & 87.1 & 96.4 & 97.6 & 98.6 \\
0 & 79.8 & 92.9 & 94.9 & 96.3 & 83.2 & 94.7 & 96.2 & 97.6 \\
%1 & 82.7 & 94.0 & 95.6 & 96.8 & 87.1 & 96.4 & 97.6 & 98.6 \\
1 & 83.4 & 94.5 & 96.0 & 97.0 & 87.6 & 96.6 & 97.8 & 98.6 \\
%2 & 86.1 & 96.0 & 97.1 & 98.0 & 88.3 & 97.1 & 98.2 & 98.8 \\
2 & 86.3 & 96.1 & 97.3 & 98.1 & 88.2 & 97.2 & 98.1 & 98.8 \\
%3 & 86.5 & 96.4 & 97.4 & 98.3 & 88.7 & 97.6 & 98.2 & 98.9 \\
3 & 87.2 & 96.8 & 97.9 & 98.5 & 88.8 & 97.7 & 98.4 & 99.0 \\
%4 & 87.1 & 96.8 & 97.4 & 98.4 & 88.8 & 97.6 & 98.6 & 99.1 \\
4 & 87.1 & 97.0 & 97.9 & 98.6 & 88.4 & 97.6 & 98.4 & 99.0 \\
%5 & 86.8 & 96.9 & 97.9 & 98.5 & 88.5 & 97.8 & 98.6 & 99.0 \\
5 & 86.1 & 96.8 & 97.9 & 98.6 & 87.3 & 97.4 & 98.2 & 98.9 \\

\end{tabular}}
\caption{}
\vspace{0.1cm}
\label{tab:ablation_gtg_inshop}
\end{table}

%{@{}l|cccc@{}}

==> tex_files/loss_ensembles.tex <==
\begin{table}[t]
\centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}l|ccccc|ccccc|cccc@{}}
%\toprule

\textbf{} & \multicolumn{5}{c}{CUB-200-2011} & \multicolumn{5}{c}{CARS 196} & \multicolumn{4}{c}{Stanford Online Products}\\ \hline

\textbf{Loss+Ensembles} &  \\ \hline
BIER 6  \cite{DBLP:conf/iccv/OpitzWPB17} & 55.3 & 67.2 & 76.9 & 85.1 &  - & 75.0 & 83.9 & 90.3 & 94.3 &  - &  72.7 & 86.5 & 94.0  & -\\
HDC 3  \cite{DBLP:conf/iccv/YuanYZ17} &  54.6 & 66.8 & 77.6 & 85.9 & - &  78.0 & 85.8 & 91.1 & 95.1 & - & 70.1 & 84.9 & 93.2 & - \\
%DRE 48  \cite{DBLP:conf/eccv/XuanSP18} &58.9 & 69.6 & 78.4 & 85.6 &  62.1 &  84.2 & 89.4 & 93.2 & 95.5 &  71 & - & - & - & -  \\
ABE 2  \cite{DBLP:conf/eccv/KimGCLK18} &  55.7 & 67.9 & 78.3 & 85.5 & - & 76.8 & 84.9 & 90.2 & 94.0 & - & 75.4 & 88.0 & 94.7  & -  \\
ABE 8  \cite{DBLP:conf/eccv/KimGCLK18} &  60.6 & 71.5 & 79.8 & 87.4 & - & 85.2 & 90.5 & 94.0 & 96.1 &  - & 76.3 & 88.4 &  94.8 & - \\
A-BIER 6 \cite{DBLP:journals/corr/abs-1801-04815} & 57.5 & 68.7 & 78.3 & 86.2 & - &  82.0 & 89.0 & 93.2 & 96.1 &  - & 74.2 & 86.9 & 94.0 & - \\
D and C 8  \cite{DDBLP:conf/cvpr/Sanakoyeu2019} & 65.9 & 76.6 & 84.4 & 90.6 & 69.6 & 84.6 & 90.7 & 94.1 & 96.5 &  70.3 &   75.9   & 88.4 & 94.9 &90.2 \\ 
RLL 3  \cite{DBLP:conf/cvpr/WangHKHGR19} & 61.3 & 72.7 & 82.7 & 89.4 & 66.1 & 82.1 & 89.3 & 93.7 & 96.7 & 71.8 &  \textbf{79.8} & \textbf{91.3} & \textbf{96.3} & 90.4\\
\hline
\textbf{Ours 2-ensemble} & 65.8 & 76.7 & 85.2 & 91.2 & 68.5 &  86.2 & 91.6 & 95.0 & 97.1 & 72.6 & 75.9 & 88.0 & 94.5 & \textbf{91.1}\\
\textbf{Ours 5-ensemble} &  \textbf{66.9} & \textbf{77.1} & \textbf{85.4} & \textbf{91.5} & \textbf{70.0} &  \textbf{88.0} & \textbf{92.5} & \textbf{95.7} & \textbf{97.5} & \textbf{74.2} &  76.3 & 88.3 & 94.6 & \textbf{91.1} \\ %\bottomrule
\end{tabular}}
\caption{Retrieval and Clustering performance of our ensemble compared with other ensemble and sampling methods. Bold indicates best results. }
\label{tab:loss_ensembles}
\end{table}
